Agile Modeling: From Concept to Classifier in Minutes

The application of computer vision to nuanced subjective use cases is growing. While crowdsourcing has served the vision community well for most objective tasks (such as labeling a "zebra"), it now falters on tasks where there is substantial subjectivity in the concept (such as identifying "gourmet tuna"). However, empowering any user to develop a classifier for their concept is technically difficult: users are neither machine learning experts, nor have the patience to label thousands of examples. In reaction, we introduce the problem of Agile Modeling: the process of turning any subjective visual concept into a computer vision model through a real-time user-in-the-loop interactions. We instantiate an Agile Modeling prototype for image classification and show through a user study (N=14) that users can create classifiers with minimal effort under 30 minutes. We compare this user driven process with the traditional crowdsourcing paradigm and find that the crowd's notion often differs from that of the user's, especially as the concepts become more subjective. Finally, we scale our experiments with simulations of users training classifiers for ImageNet21k categories to further demonstrate the efficacy.

==> Agile Modeling - arxiv/sections/0_abstract.tex <==
% Real-world applications of image classification are often triggered by a user, or ``domain expert", who wants to scale their ability to identify a particular concept.
% However, such users are usually not machine learning experts, and often have to delegate the problem to an engineer.
%Image classification is often used for a particular application or domain.  These users are often marginalized in traditional machine learning approaches, and we argue that they should be at the center of the modeling process.


The application of computer vision to nuanced subjective use cases is growing.
While crowdsourcing has served the vision community well for most objective tasks (such as labeling a ``zebra''), it now falters on tasks where there is substantial subjectivity in the concept (such as identifying ``gourmet tuna'').
However, empowering any user to develop a classifier for their concept is technically difficult: users are neither machine learning experts nor have the patience to label thousands of examples.
In reaction, we introduce the problem of Agile Modeling: the process of turning any subjective visual concept into a computer vision model through a real-time user-in-the-loop interactions.
We instantiate an Agile Modeling prototype for image classification and show through a user study (N=$14$) that users can create classifiers with minimal effort under $30$ minutes. 
We compare this user driven process with the traditional crowdsourcing paradigm and find that the crowd's notion often differs from that of the user's, especially as the concepts become more subjective.
Finally, we scale our experiments with simulations of users training classifiers for ImageNet21k categories to further demonstrate the efficacy.


==> Agile Modeling - arxiv/sections/1_introduction.tex <==
\vspace{-3em}
\section{Introduction}
\label{sec:intro}

% State: Data curation today is done in an objective way.
Whose voices, and therefore, whose labels should an image classifier learn from? In computer vision today, the answer to this question is often left implicit in the data collection process.
Concepts are defined by researchers before curating a dataset~\cite{deng_imagenet_2009}. 
Decisions for which images constitute positive versus negative instances are conducted by majority vote of crowd workers annotating this pre-defined set of categories~\cite{lease2011quality,sheng2008get}.
An algorithm then trains on this aggregated ground truth, learning to predict labels that represent the crowd's majoritarian consensus.

% Problem: People want classifiers for subjective concepts.
As computer vision matures, its application to nuanced, subjective use cases is burgeoning.
While crowdsourcing has served the vision community well on many objective tasks (e.g.~identifying ImageNet~\cite{deng_imagenet_2009} concepts like ``zebra'', ``tiger''),  it now falters on tasks where there is substantial subjectivity~\cite{gordon2021disagreement}.
Everyday people want to scale their own decision-making on concepts others may find difficult to emulate: for example, in Figure~\ref{fig:concept-images}, a sushi chef might covet a classifier to source gourmet tuna for inspiration. Majority vote by crowd workers may not converge to the same definition of what makes a tuna dish gourmet.

% While this prescribed procedure has served the vision community well on many objective tasks (e.g.~identifying ImageNet concepts like ``zebra'', ``tiger''),  it now runs aground on tasks where there is substantial subjectivity on whether an instance is undoubtedly positive or negative~\cite{gordon2021disagreement}.
% As computer vision as matured, its application to nuanced personalized use cases is burgeoning.
% Users want their personal classifiers to augment their workflows:
% a sushi chef might covet a classifier to source gourmet tuna for their omakase;
% a fashionista might want to identify flared casual pants that are currently running amok amongst the new generation.
% A majoritarian interpretation of crowd labels can not decide what a makes a tuna gourmet nor which pants are casual.

\begin{figure}[t]
  \centering
%   \hspace*{-0.5cm}                                         \vspace{-1ex}          
   \includegraphics[width=\linewidth]{img/pull_figure_hat.pdf}
%   \vspace{-4ex}
   \caption{Visual concepts can be nuanced and subjective, differing from how a majoritarian crowd might label a concept. For example, a graduate student may think that well-prepared tuna sandwiches are considered \texttt{gourmet tuna}, but sushi chef might disagree.
   }
   \label{fig:concept-images}
    \vspace{-1em}
\end{figure}

% Challenge 1: concepts are subjective and don't have an agreed upon definition. Users need to be directly involved in the data curation process.
% Challenge 2: diversity of occurrences is hard to account for apriori and needs to be iteratively defined
% Challenge 3: most users are not machine learning experts and there is a dearth of systems that makes interactions intuitive and easy for anyone to use.
This paper highlights the need for user-centric approaches to developing real-world classifiers for these subjective concepts.
To define this problem space, we recognize the following challenges. First, concepts are subjective, requiring users to be embedded in the data curation process. 
Second, users are usually not machine learning experts; we need interactive systems that elicit the subjective decision boundary from the user. 
Third, users don't have the patience nor resources to sift through the thousands of training instances that is typical for most image classification datasets~\cite{deng_imagenet_2009,lin2014microsoft,openimages}—for example, ImageNet annotated over 160M images to arrive at their final 14M version.

% The Agile Modeling problem: What is it at a high level.
In order to tackle these challenges, we introduce the problem of \textbf{Agile Modeling}: the process of turning any visual concept into a computer vision model through a real-time user-in-the-loop process.
Just as software engineering matured from prescribed procedure to ``agile'' software packages augmenting millions of people to become software engineers, Agile Modeling aims to empower anyone to create personal, subjective vision models.
It formalizes the process by which a user can initialize and interactively guide the training process while minimizing the time and effort required to obtain a model.
With the emergent few-shot learning capabilities of vision foundation models~\cite{radford2021learning,jia2021scaling}, now is the right time to begin formalizing and developing Agile Modeling systems. 


We instantiate an Agile Modeling prototype for image classification to highlight the importance of involving the user-in-the-loop when developing subjective classifiers. 
Our prototype allows users to bootstrap the learning process with a single language description of their concept (e.g.~``gourmet tuna'') by leveraging vision-language foundation models~\cite{radford2021learning,jia2021scaling}.
Next, our prototype uses active learning to identify instances that if labeled would maximally improve classifier performance. These few instances are surfaced to the user, who is only asked to identify which instances are positive, something they can do even without a background in machine learning.
This iterative process continues with more active learning steps until the user is satisfied with their classifier's performance.

% How does the prototype tackle the challenges laid out. End by saying that this is merely a first attempt at the problem and hope that the formalization will bring in more researchers.
% Our user studies with the prototype show that users can develop subjective classifiers for over $14$ concepts, each in under $30$ minutes. With our optimizations, each round of active learning operates over over 10M images and can be performed on a single desktop CPU in a few minutes. 
%We show that crowd workers produce classifiers that do not emulate the decision making. While our prototype is simple, it showcases the possibility of tackling the challenges associated with Agile Modeling. First, users can define subjective concepts and iteratively refine their subjective classifier. Second, they don't need any machine learning experience. Third, active learning reduces the amount of time users spend annotating.
% By formulating the problem and introducing a prototype for evaluation, we encourage more researchers to begin Agile Modeling.

Our contributions are:
\begin{enumerate}[noitemsep, topsep=0pt] 
%[leftmargin=*,noitemsep, topsep=0pt, labelwidth=!, labelindent=0pt,label=\textbf{\arabic*})]
    \item We formulate the Agile Modeling problem, which puts users at the center of the image classification process.
    \item  We demonstrate that a real-time prototype can be built by leveraging SOTA image-text co-embeddings for fast image retrieval and model training. With our optimizations, each round of active learning operates over over 10M images and can be performed on a single desktop CPU in a few minutes. In under 5 minutes, user-created models outperform zero-shot classifiers.
    \item In a setting that mimics real-world conditions, we compare models trained with labels from real users versus crowd raters. We find that the value of a user increases when the concept is nuanced or difficult.
    % \item We demonstrate how a small amount of annotated data can quickly beat zero-shot classifiers, and show that small batches are better early in the active-learning process.
    \item We verify the results of the user study with a simulated experiment of 100 more concepts in ImageNet21k.
\end{enumerate}

\begin{figure*}[!t]
  \centering
   \vspace{-3ex}
   \includegraphics[width=\textwidth]{img/system.pdf}
   \vspace{-2em}
   \caption{Overview of the Agile Modeling framework. Starting with a concept in the mind of the user, the system guides the user into first defining the concept through a few text phrases, automatically expands these to small subset of images, followed by one or more rounds of real-time active learning on a large corpus, where the user only needs to rate images.
   }
   \label{fig:system}
\end{figure*}
%   \rk{This needs more information. Readers should be able to read just the captions of the paper and absorb all the main takeaways.}

==> Agile Modeling - arxiv/sections/2_related_work.tex <==

% \kenji{I also feel there is some missing related work on ``in the wild" classification. Here are some pointers:
% \begin{enumerate}
%     \item \url{https://arxiv.org/pdf/1709.01450.pdf}
%     \item \url{https://openaccess.thecvf.com/content_cvpr_2016/papers/Zhu_Traffic-Sign_Detection_and_CVPR_2016_paper.pdf}
% \end{enumerate}
% }

\section{Related work}
\label{sec:related-work}
Our work draws inspiration from human-in-the-loop, personalization, few-shot, and active learning.
% We now discuss related work on human-in-the-loop computation, personalized computer vision, and zero and few-shot learning.

%Agile Modeling builds upon previous work in zero and few-shot learning, active learning, and semi-supervised learning in order to train image classifiers through human-in-the-loop interfaces.

%We now present related work in a variety of areas, including human-in-the-loop computation, zero- and few-shot learning and active learning. 

\vspace{1ex}
\noindent\textbf{Building models with humans-in-the-loop.}
Involving humans in the training process has a long history in crowdsourcing~\cite{fails2003interactive,amershi2014power,patel2010gestalt,fiebrink2009play}, in developmental robotics~\cite{thomaz2008teachable,knox2013learning,loftin2016learning}, and even in computer vision~\cite{krishna2022socially,daum2022vocal,zhang2023equi,krishna2021visual,park2019ai} and is recently all the rage in large language modeling~\cite{ouyang2022training}.
However, all these methods are primarily focused on improving model behavior. In other words, they ask ``how can we leverage human feedback or interactions to make a better model?'' In comparison, we take a user-centric approach and ask, ``how can we design a system that can empower users to develop models that reflect their needs?'' 

With this framing in mind, our closest related work belongs comes from the systems community~\cite{tropel, Snorkel, varma2017inferring, Mullapudi}.
Tropel~\cite{tropel} automated the process of large-scale annotation by having users provide a single positive example; and asking the crowd to determine whether other images are similar to it.
For subjective concepts, particularly those with multiple visual modes, a single image may be insufficient to convey the meaning of the concept to the crowd.
Others such as Snorkel~\cite{Snorkel, varma2017inferring} circumvented large-scale crowd labeling through the use of expert-designed labeling functions to automatically annotate a large, unlabeled dataset.
However, in computer vision, large datasets of images contain metadata that is independent of the semantics captured within the photo~\cite{thomee2016yfcc100m}.
% Perhaps the closest work to ours is Mullapudi et al.~\cite{Mullapudi}, which demonstrates a method of interleaving model training and expert labeling phases to build classifiers for rare concepts.  
With the recent emergent few-shot capabilities in large vision models, its now time to tackle the human-in-the-loop challenges through a modeling lens appropriate for the computer vision community.
Our prototype can train a model using active learning on millions of images on a single CPU in a matter of minutes.
% We differ from this work in several ways. In that paper, an expert is simulated by incrementally revealing the ground truth labels of images from datasets such as iNaturalist~\cite{iNaturalist} and Places~\cite{Places}. In contrast, we build a system that truly accommodates a real user.
% While~\cite{Mullapudi} focuses on rare fine-grained categories, the concepts themselves are pre-defined by the existing benchmarks rather than proposed by actual users. The universe of unlabeled examples is taken from the training set of the benchmarks themselves, making it impossible to find interpretations of a concept beyond what is available there. In contrast, we  use a large unlabeled dataset (LAION-400M~\cite{schuhmann2021laion}) to enable the users to explore and define the boundaries of their concept as they interact with the system and, in some cases, discover or clarify visual modes of the concept through this interaction.
% While Mullapudi et al~\cite{Mullapudi} require users to provide at least a few positive examples to train a classifier, our method obviates this requirement by allowing users to find related images by describing their concept in words.
% Finally, we present a detailed comparison of our user centered approach with a traditional crowdsourcing-based one.

\vspace{1ex}
\noindent\textbf{Personalization in computer vision.}
Although personalization~\cite{khan2021personalizing, cohen2022my, gal2022image} is an existing topic in building classification, detection, and image synthesis, these methods are often devoid of real user interactions, and test their resultant models on standard vision datasets. Conversely, we run a study with real users, focus on real-world sized datasets and on new, subjective concepts.

\vspace{1ex}
\noindent\textbf{Zero and few-shot learning.}
Since users have a limited patience for labeling, Agile Modeling aims to minimize the amount of labeling required, opting for few-shot solutions~\cite{metadataset, vinyals2016matching, shen2017deep, chen2020big, mullapudi2021background}.
Luckily, with the recent few-shot properties in vision-language models (found for example in CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}), it is now possible to bootstrap classifiers with language descriptions~\cite{pratt2022does}. 
Besides functioning as a baseline, good representations have shown to similarly bootstrap active learning~\cite{tian2020rethinking}.
We demonstrate that a few minutes of annotation by users can lead to sizeable gains over these zero-shot classifiers.

\vspace{1ex}
\noindent\textbf{Real-time active learning.}
% \cite{shen2017deep} shows how active learning can be used on deep learning datasets to reduce the training set size to 25\% of original, while matching performance.
% \cite{coleman2022similarity} enables "web-scale" active learning by restricting labeling candidates to the nearest neighbors of the currently labeled set instead of scanning over all of the unlabeled data. 
Usually few-shot learning can only get you so far, especially for subjective concepts where a single language description or a single prototype is unlikely to capture the variance in the concept. Therefore, iterative approaches like active learning provide an appropriate formalism to maximize information about the concept while minimizing labels~\cite{al_survey,Chuang}. 
Active learning methods derive their name by ``actively'' asking users to annotate data which the model currently finds most uncertain~\cite{uncertainty} or believes is most representative of the unlabeled set~\cite{sener2017active} or both~\cite{ash2019deep,citovsky2021}.
Unfortunately, most of these methods require expensive pre-processing, reducing their utility in most real-world applications~\cite{daum2023vocalexplore}. Methods to speed up active learning limit the search for informative data points~\cite{coleman2022similarity} or use low-performing proxy models for data selection~\cite{coleman2019selection} or use heuristics~\cite{sener2017active, pinsler2019bayesian}.
We show that performing model updates and ranking images on cached co-embedding features is a scalable and effective way to conduct active learning.

%\vspace{-1em}

==> Agile Modeling - arxiv/sections/3_agile_system.tex <==
\section{Agile Modeling}
\label{sec:system}

A user comes to the Agile Modeling system with just a subjective concept in mind---in our running example, \concept{gourmet tuna}. First we lay out the high level Agile Modeling problem framework and then describe how we instantiate a prototype of this framework.

\subsection{The framework}
As shown in Figure~\ref{fig:system}, the Agile Modeling framework guides the user through the creation of a image classifier through the following steps:
\setul{3pt}{.4pt}
\begin{enumerate}[noitemsep] 
    \item \ul{Concept definition.} The user describes the concept using text phrases. They are allowed to specify both positive phrases, which can describe the concept as a whole or specific visual modes, as well as negative phrases, which are related but not necessarily part of the concept (\eg \concept{canned tuna} is not gourmet).
    \item \ul{Text-to-image expansion and image selection.} The text phrases are used to mine relevant images from a large unlabeled dataset of images for the user to rate.
    \item \ul{Rating.} The user rates these images through a rating tool, specifying whether each image is either \texttt{positive} or \texttt{negative} for the concept of interest.
    \item \ul{Model training.} The rated images are used to train a binary classifier for the concept. This is handled automatically by the system.
    \item \ul{Active learning.} The initial model can be improved very quickly via one or more rounds of active learning. This consists of 3 repeated steps: (1) the framework invokes an algorithm to select from millions of unlabeled images to rate; (2) the user rates these images; (3) the system retrains the classifier with all the available labeled data. The whole active learning procedure operates on millions of images and returns a new model in under 3 minutes (measured in Section~\ref{sec:obtaining-model-in-minutes}).
    %\item \underline{Active Learning with Crowd Raters.} When we finish performing AL with the expert in the loop, either because the model is good enough or because the user cannot spend more time, we can optionally iterate through more AL rounds with crowd raters.
\end{enumerate}

The user's input is used for only two types of tasks, which require no machine learning experience: first in providing the text phrases and second in rating images. Everything else, including data selection and model training, is performed automatically. With such an automated process, users do not need to hire an machine learning or computer vision engineer to build their classifiers.

% Once the user has obtained a model, the system also provides the option of continuing the active learning loop with crowd raters (from a crowdsourcing platform) instead of the user, if desired. In order to use the crowdsourcing platform, the user is required to provide guidelines describing the concept.
%Additionally, our formulation allows for a seamless transition between user and crowd-raters. 


\subsection{The prototype}
We focus our prototype on the core north star task of image classification~\cite{fei2022searching}. One of the main challenges of Agile Modeling is to enable the user to effectively transfer their subjective interpretation of a concept into an operational machine learning model. For our image classification task, Agile Modeling seeks to turn this arbitrary concept into a well-curated training dataset of images. We assume that that the user only has access to a large, unlabeled dataset, which is something that is easily available through the internet~\cite{radford2021learning}. Our aim is to select and label a small subset of this large dataset and use it as training data.

\vspace{1ex}
\noindent\textbf{Concept definition.}
Users initiate the Agile Modeling process by expressing their concept in words. For example, the user might come in and simply say \concept{gourmet tuna}.
However, users can preemptively also provide more than a single phrase. They can also produce negative descriptions of what their concept is \textit{not}. They can clarify that \concept{canned tuna} is not gourmet.
Through our interactions with users, we find that expressing the concept in terms of both positive and negative phrases is an effective way of mining positive and hard negative examples for training.
The positive phrases allow the user to express both the concept as a whole (\eg \concept{gourmet tuna}) and specific visual modes of it (\eg \concept{seared tuna}, \concept{tuna sushi}). The negative phrases are important in finding negative examples that could be easily confused by raters.

% To do so, we mine images,  as described in Section~\ref{sec:query-expansion},  by leveraging the concept definition phase where the user 
% There different ways to request this input, for instance a paragraph describing the full meaning of the concept. However,
 
\vspace{1ex}
\noindent\textbf{Text-to-image expansion and image selection.}
\label{sec:query-expansion}
The phrases provided by the user are used to identify a first set of relevant training images. To achieve this, we take advantage of recent, powerful image-text models, such as CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}. We co-embed both the unlabeled image dataset and the text phrases provided by the user into the same space, and perform a nearest-neighbors search to retrieve 100 images nearest to each text embedding. We use an existing nearest-neighbors implementation~\cite{wu2017multiscale, guo2016quantization} that is extremely fast due to its hybrid solution of trees and quantization. From the set of all nearest neighbors, we randomly sample 100 images for the user to rate. We do this for both positive and negative phrases, since the negative texts are helpful in identifying hard negative examples.

% \subsection{Image selection}
% \label{sec:image-expansion}
% Out of the images expanded from the phrases, we randomly select a small subset (on the order of 100) which we ask the user to rate.


% Why not directly retrieve 100 images from the text expansion? We found that expanding to the immediate nearest neighbors of the text phrases will yield images which are very similar to each other or even near duplicates. On the other hand, expanding to a larger subset, followed by random down-sampling brings in much needed diversity. In fact, this step is crucial in the performance of the final classifier, because once a visual mode is missed---that is, the model classifies one special case of our concept as negative---it will be hard for any future steps, including active learning, to recover it.

% We found that first expanding the phrases to more images and then carefully selecting a subset leads to a better initial model. That's because our selection strategy, which we introduce next, makes smart use of the limited labeling budget: it selects diverse images, covering various visual modes, while avoiding the selection of near-duplicate images. In fact, this step is crucial in the performance of the final classifier, because once a visual mode is missed -- that is, the model classifies one of the special cases of our concept as negative -- it will be hard for any future steps, including active learning, to recover it.

% \paragraph{Graph-based diversity sampling. } To choose a diverse set of samples from the expansion pool, we first build a similarity graph with images as the nodes. If the similarity measure of two images is larger than a given threshold, we connect them with an edge. We define the similarity of two images as the cosine of their corresponding vectors in the feature space. Intuitively, two nodes that are neighbors of each other do not both need to be sampled, as one likely "covers" the other in the underlying feature space.  A node is covered if the node itself or its neighbor is sampled. We aim to select a subset of the graph such that the coverage is maximum for the given sampling budget. This problem can be reduced to the Set Cover optimization problem and solved with algorithms introduced in ~\cite{bateni2017almost, bateni2018optimal}. Our approximation to solve this NP-hard problem is to sample the nodes based on their degree, selecting the highest degree node first. Once a node is sampled, the node itself and all of its neighbors are removed from the graph. This process is iterated until the desired number of nodes are selected. If the graph is covered before the budget is exhausted, we continue to randomly sample from the graph to exhaust the budget. Using maximal coverage sampling on the graph has several advantages. Firstly, we avoid sampling near duplicates and therefore spend the budget more efficiently. Furthermore, different visual modes of the same concept are expected to be disjoint component of the graph, therefore maximizing the coverage makes it more likely to sample from every different visual mode of the concept. Lastly, we likely choose the most representative image of each kind, since the selected image perhaps has the most number of neighbors.

\vspace{1ex}
\noindent\textbf{Data labeling by user.} 
The selected images are shown to the user for labeling. In our experiments, we created a simple user interface where the user is shown one image at a time and is asked to select whether it is \texttt{positive} or \texttt{negative}. The median time for our users to rate a single image was $1.7 \pm 0.5$ seconds. Since users rate 100 images per annotation round, they spend approximately 3 minutes before a new model is trained.

\vspace{1ex}
\noindent\textbf{Model training.}
We train our binary image classifier using all previously labeled data. This setup is challenging because there is little data available to train a generalizable model, and the entire training process must be fast to enable real-time engagement with the user waiting for the next phase of images.
The lack of large-scale data suggests the use of few-shot techniques created to tackle low data scenarios, such as meta-learning~\cite{wang2020generalizing, hochreiter2001learning, finn2017model} or prototype methods~\cite{snell2017prototypical}, however most such approaches are too slow for a real-time user interaction.
While the study of real-time few-shot methods is an interesting problem for future instantiations of the Agile Modeling framework, we adopted another solution that helps us address both challenges: we again take advantage of powerful pretrained models like CLIP and ALIGN to train a small multilayer perceptron (MLP), with only 1-3 layers, on top of image embeddings provided by such large pretrained models. These embeddings bring much needed external information to address the low data challenge while allowing us to train a low-capacity model that can be trained fast and is less prone to overfitting. Model architectures and training details are described in Section~\ref{sec:experiments}.

\vspace{1ex}
\noindent\textbf{Active learning (AL).}
\label{sec:al}
We improve the classifier in the traditional model-based active learning fashion: (1) we use the current model to run inference on a large unlabeled pool of data, (2) we carefully select a batch of images that should be useful in improving the model, (3) we rate these images, (4) we retrain the model. This process can be repeated one or more times to iteratively improve performance. 
% There are some of important questions to be decided: who is doing the rating, and what algorithm we should use for sample selection.
% \vspace{1ex}
% \textbf{AL with user vs crowd raters.} Although the user provides the highest-quality labeling for AL, in many real-world scenarios users have limited time, so they cannot spend hours rating data. We could delegate rating---either in part or entirely---to crowd workers. The user may do a few rounds of AL (constrained by their availability), which can then be continued with zero or more rounds of crowd-based AL (constrained by the rating budget). Aside from the time and money constraints, there is one more consideration specific to the Agile Modeling setting: only the users know the full meaning of the concept, while crowd-workers can easily make mistakes or wrong assumptions about the concept, leading to noisier data. This effect may be less visible on benchmark datasets like ImageNet, where the concepts are more factual (\eg detecting specific objects or breeds of animals). However, Agile Modeling gives users the possibility of creating models for any kinds of concepts, no matter how ambiguous or personalized they may be. In such cases, crowd raters may make mistakes at even higher rates. In our experiments we study the trade-offs between user and crowd.
% \paragraph{Weighted Max-Cover algorithm.} Ideally we would want to pick a state-of-the-art AL method that can improve the model fastest. However, when the user is the rater, we have a real-time constraint: we need the AL method to make its sample selection very fast, to make the best use of the user time and offer them a pleasant user-interaction with our system. Therefore, AL methods that rely on heavy optimization strategies {\color{red} [TODO: cite some]} cannot be used. A solution that is fast and has been shown to perform well is {\em margin sampling} {\color{red} [cite]}, which is one of the methods tested in our experiments. However, inspired by the success of diversity sampling for the initial pool selection, we introduce another strategy that provides an improvement over margin sampling and is real-time.
% We introduced our graph-based diverse sampling algorithm in {\color{red} section XXXXX}. To leverage the trained model in our sampling we use the weighted version of maximal coverage as described in ~\cite{bateni2018optimal} for sampling from the 2500 shortlisted candidates. In this algorithm a weight is associated with each node (image) and the objective is to maximize the total weight of covered nodes. We use one minus the margin score of each image as its weight. The node weights are then multiplied by the incoming edge weights (similarity) and aggregated. This score is used as the marginal benefit of including a node in the sampled subset.
When selecting samples to rate, state-of-the-art AL methods generally optimize for improving the model fastest~\cite{ren2021survey}. However, when the user is the rater, we have a real-time constraint to minimize the user-perceived latency. Therefore, AL methods that rely on heavy optimization strategies cannot be used. In our solution, we adopt a well-known and fast method called {\em uncertainty sampling} or {\em margin sampling}~\cite{culotta2005reducing, scheffer2001active, lewis1995sequential}, which selects images for which the model is {\em uncertain}. Specifically, given a model with parameters $\theta$ and a sample $x$, we define the uncertainty score as $ P_{\theta}(\hat y_1|x) -  P_{\theta}(\hat y_2|x)$, where $\hat y_1$  and $\hat y_2$ are the highest and second-highest probabilities predicted by the model.
% \textbf{(i)} $1 - P_{\theta}(\hat y|x)$, where $\hat y$ represents the highest posterior probability predicted by the model---in other words, this selects samples where the highest prediction is not confident;
% \textbf{(ii)} $\sum_{i \in \{0,1\}} P_{\theta}(\hat y_i|x) \log P_\theta(\hat y_i|x)$, which this selects the samples with the highest entropy;
%\textbf{(iii)} $ P_{\theta}(\hat y_1|x) -  P_{\theta}(\hat y_2|x)$, where $\hat y_1$  and $\hat y_2$ are the highest and second-highest probabilities predicted by the model.
Note there are other definitions of uncertainty such as least confidence and entropy, but since we are in a binary classification setting, all of these definitions are mathematically equivalent. 
% We also consider the approach adopted by \cite{Mullapudi}, which is a combination of margin and positive mining. In each AL round, the rating phase is divided into sub-rounds, where in each sub-round samples are selected based on one of two strategies: if so far we have rated more positives than negatives, we select samples from the margin, otherwise we pick samples with the highest prediction scores (to mine for positives). We compared both margin and this approach in our experiments.
We run one or more rounds of AL, the number of rounds is determined by the time the user has.
%and the performance of the model (once the model performance starts converging, we can stop).

==> Agile Modeling - arxiv/sections/4_experiments.tex <==
\section{Experiments with real users}
\label{sec:experiments}

We run user studies with real users in the loop, and show that:
\textbf{(1)} In only 5 minutes, the performance of an Agile model can exceed that of state-of-the-art zero-shot models based on CLIP and ALIGN by at least $3\%$ AUC PR (Section~\ref{sec:obtaining-model-in-minutes});
\textbf{(2)} For hard, nuanced concepts, Agile models trained with user annotations outperform those trained with crowd annotations even when crowd raters annotate 5x more data (Section~\ref{sec:value-of-domain-experts});
\textbf{(3)} Smaller active learning batch sizes perform better than larger ones, but there is an efficiency trade-off (Section~\ref{sec:ablation});
\textbf{(4)} Agile models using ALIGN embeddings outperform does using CLIP throughout model iterations (Section~\ref{sec:ablation});

\subsection{Choosing subjective concepts}

\vspace{1ex}
\noindent\textbf{Concepts.} For our user studies we select a list of $14$ novel concepts, spanning different degrees of ambiguity and difficulty. The list ranges from more objective concepts such as \concept{pie chart}, \concept{in-ear headphones} or \concept{single sneaker on white background}, to more subjective ones such as \concept{gourmet tuna}, \concept{healthy dish}, or \concept{home fragrance}. 
We found that our concepts cover a large spread over the visual space; we measure this spread using the average pairwise cosine distance between the concept text embeddings (using CLIP). For our $14$ concepts, the average pairwise cosine distance was $0.73 \pm 0.13$. In comparison, ImageNet's average pairwise cosine distance was $0.35 \pm 0.11$.
The full list of concepts is included in Appendix~\ref{appendix:concepts}, along with the queries provided by the users.

\vspace{1ex}
\noindent\textbf{Workflow.} We provide users with only the concept name and a brief description, but allow them to define the full interpretation. 
For instance, one of our users, who was provided with the concept \concept{stop-sign}, limited its interpretation to only real-world stop-signs: only stop signs in traffic were considered positive, while stop-sign drawings, stickers, or posters were considered negative\footnote{This definition was inspired by a self-driving car application, where a car should only react to real stop signs, not those on posters or ads.}.

% \begin{table}
%   \centering
%   \small
% %   \setlength{\tabcolsep}{2pt}
% %   \lato
%   \begin{tabular}{lccc}
%     \toprule
%     Setting & AUC PR & AUC ROC & F1  \\
%     \midrule
%     zero-shot               & 54.7 $\pm$ 2.7 & 64.2 $\pm$ 1.0 & 18.8 $\pm$ 4.7 \\ 
%     crowd only              & 64.7 $\pm$ 0.6 & 70.5 $\pm$ 0.4 & 47.8 $\pm$ 1.0 \\
%     crowd only ($\times 5$) & X $\pm$ Y & X $\pm$ Y & X $\pm$ Y\\
%     expert only             & \textbf{69.3 $\pm$ 2.4} & \textbf{72.9 $\pm$ 1.3} & \textbf{58.2 $\pm$ 2.0} \\
%     \bottomrule
%   \end{tabular}
%   \vspace{-1ex}
%   \caption{Final model performance ($\%$), mean and standard deviation over all concepts for the zero-shot baseline, crowd-only baseline, crowd with 5 times as much rating per active learning round, and our domain-expert only method.}
%   \label{tab:final-model-performance}
% \end{table}

\begin{table}
  \centering
  \small
  \vspace{-1ex}
  \begin{tabular}{l|r}
    \toprule
    \multicolumn{1}{c|}{Step} & \multicolumn{1}{c}{Time}  \\
    \midrule
    User rates 100 images & 2 min 49 sec $\pm$ 58 sec\\
    AL on 10M images & 58.6 sec $\pm$ 0.8 sec \\
    Training a new model & 23.1 sec $\pm$ 0.2 sec\\
    \bottomrule
  \end{tabular}
  \vspace{-1ex}
  \caption{The average and standard deviation of the time it takes per step in our Agile Modeling instantiation. Rating time was measured by taking the average median time of an user to rate one image during the experiments used in this paper. To measure time for AL and model training, they were each run 10 times.}
  \label{tab:time-per-step}
  \vspace{-1em}
\end{table}


\vspace{1ex}
\noindent\textbf{Participants.} When collecting data for the experiments, we sourced $14$ volunteer users to interact with our system. Each participant built a different concept. None of the users performed any machine learning engineering tasks. Our experiments indicate that it takes participants $2$ minutes and $49$ seconds on average to label $100$ images, as shown in Table~\ref{tab:time-per-step}. Our participants were adults that spanned a variety of age ranges (18-54), gender identities (male, female), and ethnicities (White, Asian, and Middle Eastern).

\vspace{1ex}
\noindent\textbf{Data sources.} Since our prototype requires an unlabeled source of images from which to source training labels, we use the LAION-400M dataset~\cite{schuhmann2021laion}, due to its large size and comprehensive construction based on the large Common Crawl web corpus. We throw away the text associated with the images. We remove duplicate URLs and split imags into a $100$M training and $100$M testing images. All Agile models trained use data exclusively from the unlabeled training split, including during nearest neighbor search, active learning, and training. For evaluation, we only use data from the $100$M test set, where each concept's evaluation set consists of a subset of this data rated by the user.
%we run inference of all models on the test set.

\subsection{Experimental setup}
\label{sec:experimental_setup}

\textbf{Models and training.}
All models are multilayer perceptrons (MLP) that take image representations from a frozen pretrained model as input and contain one or more hidden layers. For the first active learning step, we use a smaller MLP with $1$ hidden layer of $16$ units to prevent overfitting, while all active learning rounds and final model have $3$ hidden layers of size $128$. 
All training details, including optimizer, learning rate, etc., can be found in Appendix~\ref{appendix:experimental-details}.
% All models are trained using binary cross-entropy loss, a dropout rate of 0.5 and weight decay regularization with weight \num{1e-4}. We use the Adam optimizer \cite{adam} with learning rate \num{1e-4} and train for 10 epochs. To prevent overtriggering by the trained classifier, we sample 500k random images from the unlabeled set and automatically label them negative. During training, we upsample our labeled positives to be half the training set, while labeled negatives and the random negatives are each a quarter of the training set. All hyperparameters have been chosen on 2 held-out concepts.

\vspace{1ex}
\noindent\textbf{Baselines.}
One baseline we compare against is zero-shot learning, which corresponds to zero effort from the user. We implement a zero-shot baseline that scores an image by the cosine similarity between the image embedding and the text embedding of the desired concept. 
% For evaluation metrics that require binary predictions, we classify an image as positive if the cosine similarity exceeds a certain threshold. When using CLIP, we chose the threshold to be 0.28, based on LAION-5B's human inspection~\cite{schuhmann2022laion}. We similarly chose 0.2 as a threshold when using ALIGN based on our own inspection.
We also compare against a recently released active learning algorithm for learning rare vision categories~\cite{Mullapudi}. This system is the most relevant related work. We replace our active learning algorithm with theirs and compare the performance in Section~\ref{sec:ablation}.
% Ideally we would compare ours systems end-to-end, however, the code of \cite{Mullapudi}'s system has not been released along with the publication, and we also believe that it cannot be reimplemented to run in real-time on a CPU, because it requires fine-tuning large (???) ResNet models. 
% Therefore, we only reimplemented their active learning algorithm and compared against it in \Cref{experiments:stanford}}.


\begin{figure}[t]
  \centering
  \vspace{-1ex}
   \includegraphics[width=\linewidth]{plots/zsBaseAlign_results_per_num_samples_auc_pr_zsBaseClipAlign.pdf}
   \vspace{-1.5em}
   \caption{Model performance per amount of samples rated by the user (AUC PR mean and standard error over all concepts). Each $\bullet$ corresponds to an active learning round.}
   \label{fig:zs-vs-base-auc-pr}
  \vspace{-1em}
\end{figure}



\begin{figure*}[t]
     \centering
     \vspace{-2ex}
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \vspace{-1ex}
         \includegraphics[width=\linewidth]{plots/user-crowd_results_per_num_samples_auc_pr_baseCrowd_hardest7Zs.pdf}
         \caption{Hard concepts -- per \# samples rated}
         \label{fig:al-auc-pr-crowd-hardest-per-sample}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \vspace{-1ex}
         \includegraphics[width=\linewidth]{plots/user-crowd_results_per_num_samples_auc_pr_baseCrowd_easiest7Zs.pdf}
         \caption{Easy concepts -- per \# samples rated}
         \label{fig:al-auc-pr-crowd-easiest-per-sample}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\linewidth}
         \centering
         \vspace{-1ex}
         \includegraphics[width=\linewidth]{plots/user-crowd_results_per_num_samples_auc_pr_baseCrowd.pdf}
         \caption{All concepts -- per \# samples rated}
         \label{fig:al-auc-pr-crowd-all-per-sample}
     \end{subfigure}
     % Comment the next 3 subfigures to remove row 2
    %  \begin{subfigure}[b]{0.33\linewidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{plots/crowd_results_per_al_round_auc_pr_baseCrowd_hardest7Zs.pdf}
    %      \caption{Hard concepts -- per AL round}
    %      \label{fig:al-auc-pr-crowd-hardest-per-round}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.33\linewidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{plots/crowd_results_per_al_round_auc_pr_baseCrowd_easiest7Zs.pdf}
    %      \caption{Easy concepts -- per AL round}
    %      \label{fig:al-auc-pr-crowd-easiest-per-round}
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.33\linewidth}
    %      \centering
    %      \includegraphics[width=\linewidth]{plots/crowd_results_per_al_round_auc_pr_baseCrowd.pdf}
    %      \caption{All concepts -- per AL round}
    %      \label{fig:al-auc-pr-crowd-all-per-round}
    %  \end{subfigure}
    
     \vspace{-1ex}
     \caption{Performance per \# samples rated by the user or crowd. AUC PR mean and standard error over subsets of concepts: hardest for the zero-shot model (left), easiest for the zero-shot model (middle), all (right). Each $\bullet$ represents an AL round.
        % \rk{I find the bottom row really weird. The x-axis doesn't make sense. You can either measure participant effort or measure time taken for annotation. But, an active learning step is either. crowd-500 presumable takes $5\times$ more time and effort than crowd-100 but is incomparable in terms of time to participant, who might in some cases be faster and in others slower. And while you can compare domain-expert to crowd-100 in terms of the number of labels produced, you can't compare them to crowd-500. If you want to keep the bottom row, I suggest dropping crowd-500 and just changing the x-axis to number of samples rated. It would be a zoomed in version of the graph in the top row.}
        %  When training models with crowd-rated data, one has to annotate $5$ times as much data to get comparable performance with models trained by data rated by only the participant.
        }
        \label{fig:al-auc-pr-crowd}
\end{figure*}

\begin{figure*}[t]
  \centering
  \vspace{-1ex}
   \includegraphics[width=\linewidth]{plots/zsBaseAlign_results_concept_auc_pr_squished.pdf}
   \vspace{-2.2em}
   \caption{Model performance per concept for zero-shot and user-in-the-loop Agile models on CLIP and ALIGN embeddings.}
     \vspace{-1ex}
   \label{fig:results_per_concept-auc-pr}
\end{figure*}



\vspace{1ex}
\noindent\textbf{Evaluation protocol.} To evaluate the models trained with the Agile Modeling prototype, we require an appropriate test set. Ideally, the user would provide a comprehensive test set---for example, ImageNet holds out a test set from their collected data~\cite{russakovsky2015imagenet}. However, since our users are volunteers with limited annotation time, they cannot feasibly label the entire LAION-400M dataset or its $100$M test split. Additionally, since we are considering rare concepts, labeling a random subset of unlabeled images is unlikely to yield enough positives.
To address these problems, we ran stratified sampling on each model, which divides images based on their model score into $10$ strata ranging from $[0,0.1)$ to $[0.9,1.0]$. In each strata, we hash each image URL to a 64-bit integer using the pseudorandom function SipHash~\cite{aumasson2012siphash} and include the 20 images with the lowest hashes in the evaluation set. Each model contributes equally to final test set. The final evaluation set has over $500$ images per category with approximately $50\%$ positive rate. The full details of the evaluation set distribution and acknowledgement of its potential biases can be found in Appendix~\ref{appendix:evaluation_strategy}.


\vspace{1ex}
\noindent\textbf{Other hyperparameters.} The text-to-image expansion expands each user-provided query to $100$ nearest-neighbor images. Next, the image selection stage randomly selects a total of $100$ images from all queries, leading to an initial training set of $100$ samples for the first model. Users are asked to perform $5$ rounds of active learning, rating $100$ images per step. These hyperparameters were chosen based on two held-out concepts, and the ablation results in Section~\ref{sec:ablation}.



\subsection{Results}

\subsubsection{Users produce classifiers in minutes}
\label{sec:obtaining-model-in-minutes}

A key value proposition of Agile Modeling is that the user should be able to train a model in minutes. We now report the feasibility of this proposition.



\vspace{1ex}
\noindent\textbf{Measuring Time.}
The time it takes per for each step of the framework is detailed in Table~\ref{tab:time-per-step}. Our proposed Agile Modeling implementation trains one initial model and conducts five active learning rounds, taking 24 minutes on average to generate a final model.

\vspace{1ex}
\noindent\textbf{Comparison with zero-shot.} 
We start by comparing against zero-shot classification, which corresponds to a scenario with minimal effort from the user. In  Figure~\ref{fig:zs-vs-base-auc-pr}, we present the performance our instantiations of the Agile Modeling framework against a zero-shot baseline across two image-text co-embeddings: CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}.
We find that the zero-shot  performance is roughly on par as a supervised model trained on 100 labeled examples by the user.
However, after the user spends a few more minutes rating (i.e., as the number of user ratings increases from 100 to 600), the resulting supervised model outperforms zero-shot. 
% We find that crowd labeling performs significantly worse even with larger batch sizes, highlighting the importance of userise in initializing and creating performant visual classifiers for difficult concepts. A small amount of work ($\sim$30 minute) from the user creates accurate classifiers with far fewer labels compared to larger-scale crowd labeling. We further find that using large-scale crowd labeling cooperatively with users slightly improves accuracy, suggesting that the expertise of users helps find relevant images much faster than the crowd on its own. 




% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{plots/crowd_results_per_num_samples_auc_pr_baseCrowd.pdf}
%   \vspace{-2em}
%   \caption{Model performance per amount of samples rated by the participant versus crowd. Mean and standard error over all concepts. Each $\bullet$ corresponds to an active learning round. When training models with crowd-rated data, one has to annotate $5$ times as much data to get comparable performance with models trained by data rated by only the participant.}
%   \label{fig:al-auc-pr-crowd}
% \end{figure}


\vspace{1ex}
\noindent\textbf{User time versus performance.} To measure the trade-off between user time versus model performance, we show in Figure~\ref{fig:zs-vs-base-auc-pr} the AUC PR of the model across active learning rounds. We include additional metrics in Appendix~\ref{appendix:al-results}.
We include results for both CLIP and ALIGN representations as input to our classifiers. We also compare against the respective zero-shot models using CLIP and ALIGN, which are considered the zero effort case.
For both types of representations, we see a steeper increase in performance for the first 3 active learning rounds, after which the performance starts to plateau, consistent with existing literature applying active learning to computer vision tasks~\cite{karamcheti2021mind}.
Interestingly, for CLIP representations, the initial model trained on only $100$ images performs worse than the zero-shot baseline, but the zero-shot model is outperformed with just one round of active learning. We do not see this effect on ALIGN representations, where even 100 samples are enough to outperform the zero-shot model---perhaps because ALIGN representations are more effective.
We compare CLIP and ALIGN in more detail in Section~\ref{sec:ablation}.
Importantly, We show that with only 5 minutes of the user's time (Table~\ref{tab:time-per-step}), we can obtain a model that outperforms the zero-shot baseline by at least $3\%$. After 24 minutes, this performance gain grows to 16\%.



\begin{figure}[!t]
  \centering
  \vspace{-2ex}
   \includegraphics[width=0.95\linewidth]{plots/marginStanfordFixresults_per_num_samples_auc_pr_withStanfordFix_allMinus2.pdf}
    \vspace{-1ex}
   \caption{Model performance for two active learning methods: margin and the approach of \cite{Mullapudi} (margin \& positive mining). Each $\bullet$ corresponds to an AL round. We show the AUC PR mean and standard error over all concepts.}
   \label{fig:al_stanford}
   \vspace{-3ex}
\end{figure}




\subsubsection{Value of users in the loop versus crowd workers}
\label{sec:value-of-domain-experts}

We now study the value of empowering users to train models by themselves. In particular, we address the following question: Are there concepts for which a user-centered Agile framework leads to better performance?

% \vspace{1ex}
% \noindent\textbf{Users produce more accurate classifiers for more subjective concepts.}
Users have an advantage over crowd raters in their ability to rate images according to their subjective specifications. However, this subjectivity, or ``concept difficulty'' varies by concept: if a concept is universally understood, the advantage diminishes. Conversely, complex, nuanced concepts are harder for crowd workers to accurately label. To take this into consideration, we first partition the concepts into two datasets based on their difficulty, using zero-shot performance
% (shown in \Cref{fig:results_per_concept-auc-pr})
as a proxy for concept difficulty. The $7$ concepts that admit the highest zero-shot performance are considered ``easy," while the remaining $7$ concepts are considered ``hard." The specific groups can be found in Appendix~\ref{appendix:concept-difficulty}. Notice that the ``difficult'' concepts include more subjective concepts such as \concept{gourmet tuna} (as illustrated in Figure~\ref{fig:concept-images}), or with multiple and ambiguous modes such as \concept{healthy dish}; whereas the ``easy'' concepts include simple, self-explanatory concepts such as \concept{dance} or \concept{single sneaker on white background}.

We then evaluate models trained by three sets of raters:
\begin{enumerate}[noitemsep, leftmargin=1em,topsep=0pt]
\item \texttt{User-100}: Users rate 100 images for the initial model and every AL round (total 600 images).
\item \texttt{Crowd-100}: Crowd workers rate 100 images for the initial model and every AL round (total 600 images).
\item \texttt{Crowd-500}: Crowd workers rate 500 images for the initial model and every AL round (total 3000 images).
\end{enumerate}

The only difference in the configurations above is who the raters are (user or crowd) and the total number of ratings. For crowd ratings, having clear instructions is crucial for accurate results, but obtaining them is a non-trivial task in the machine learning process~\cite{gadiraju2017clarity, dow2012shepherding}.
In this experiment, crowd workers read instructions created by the users, who noted difficult cases that they found during labeling. Details about the crowd instructions can be found in Appendix~\ref{appendix:crowd-task-design}. 

We plot the results in Figure~\ref{fig:al-auc-pr-crowd}, which shows the average performance for the ``hard'', ``easy'' and all concepts as a function of the number of rated samples, using CLIP embeddings. %(Figures~\ref{fig:al-auc-pr-crowd-hardest-per-sample} to \ref{fig:al-auc-pr-crowd-all-per-sample}).
% and number of active learning rounds (Figures~\ref{fig:al-auc-pr-crowd-hardest-per-round} to \ref{fig:al-auc-pr-crowd-all-per-round}).
Per-concept results can be found in Appendix~\ref{appendix:crowd}.
On hard concepts, models trained with users (User-100) outperform models trained with crowd raters, even when $5\times$ more ratings are obtained from the crowd (Crowd-500). This suggests that Agile Modeling is particularly useful for harder, more nuanced and subjective concepts.

\subsection{Ablation studies}
\label{sec:ablation}

% \subsubsection{Max-cover for a diverse initial dataset selection}
% Recall that we use a max-cover algorithm on the output of nearest neighbor search to select a diverse group of images for initial model training. To demonstrate the efficacy, we replace the max-cover algorithm with random sampling and find that XXXX.

% \subsubsection{Max-cover for model-based active learning}
% Recall that we use a max-cover algorithm on the top 2500 images selected by margin sampling to select a diverse group of K images for model training. To demonstrate its efficacy, we replace the max-cover algorithm with selecting the top-K results from margin sampling. We find that XXXX

% In the paper, we introduce a framework for Agile Modeling and a number of instantiations. The goal of this section is to show that those instantiations  are reasonable solutions to the Agile Modeling problem. 

Although our main contribution is introducing the problem of Agile Modeling, instantiating our prototype explores a number of design decisions. In this section, we lay out how these designs change the outcome.



\begin{figure}[!t]
  \centering
  \vspace{-2ex}
   \includegraphics[width=0.95\linewidth]{plots/batchSizes_results_per_num_samples_auc_pr_allUsers.pdf}
   \vspace{-1ex}
   \caption{Model performance during active learning with 3 AL batch sizes: small (50), medium (100), large (200). Each $\bullet$ corresponds to an AL round. We show the AUC PR mean and standard error over all concepts.}
   \label{fig:batch_sizes}
   \vspace{-3ex}
\end{figure}

\vspace{1ex}
\noindent\textbf{Active learning method.}
Throughout the paper, we instantiate the active learning component with the well-known margin method~\cite{margin_sampling}. We now compare it to the active learning method used in Mullapudi et al \cite{Mullapudi}.  We ran a version of our instantiation of the Agile framework where we replace margin with the margin+positive mining strategy chosen by \cite{Mullapudi} and described in Section~\ref{sec:al}. The performance of the two methods per AL round is shown in Figure~\ref{fig:al_stanford}. Interestingly, despite the fact that Mullapudi et al. \cite{Mullapudi} introduced this hybrid approach to improve upon margin sampling, in this setting the two methods perform similarly across all AL rounds. We see the same effect on most concepts when inspecting on a per-concept basis in Appendix~\ref{appendix:al-results}.
One potential explanation for this is that the initial model trained before AL is already good enough (perhaps due to the powerful CLIP embeddings) for margin sampling to produce a dataset balanced in terms of positive and negative, and thus explicitly mining easy positives as in~\cite{Mullapudi} is not particularly useful.
Since the two methods perform equivalently, we opted for the simpler and more efficient margin in the rest of the experiments.



\vspace{1ex}
\noindent\textbf{Active learning batch size.}
Our prototype asks the user to annotate images across $5$ rounds of active learning, $100$ images per round. However, we can simultaneously change the number of images rated per round and the number of active learning rounds the user conducts. We evaluate the downstream effects of changing active learning batch size and number of rounds on model performance and time spent. We consider $3$ batch sizes: small ($50$ images/batch), medium ($100$ images/batch), large ($200$ images/batch). We run repeated rounds of active learning with each of these settings, retraining the model after each round using CLIP representations. The results in Figure~\ref{fig:batch_sizes} show that, for a fixed amount of images rated, smaller batch sizes are better than larger, especially so in the beginning. This result is expected, because for a fixed rating budget, the smaller batch setting has the chance to update the model more frequently.
While these results suggest that we should opt for a smaller batch size, there is still a trade-off between user time and performance, even when we have the same total number of samples rated. That is because model training takes about $1$-$2$ minutes during which the user is idle, and so smaller batch sizes lead to longer time investment from the users. As a good compromise, we chose $100$ as our batch size.
% We also compared different active learning strategies in Appendix~\ref{experiments:stanford}.

\vspace{1ex}
\noindent\textbf{Stronger pretrained model improves performance.}
Since our system leverages image-text co-embeddings to find relevant images and quickly train classifiers, a logical question is: how does changing the underlying embedding change the performance of the classifier? To do this, we compare CLIP versus ALIGN as the underlying embedding by replacing our pre-cached CLIP embeddings with ALIGN. We find that, with ALIGN, the AUROC of the final Agile model increased from 0.72 to 0.80 with a relative gain of 11.5\%. The AUPR increased from 0.68 to 0.76, a relative gain of 13.1\%. Furthermore, as Figure~\ref{fig:results_per_concept-auc-pr} demonstrates, both the ALIGN zero-shot and Agile models outperform their CLIP counterparts for almost every concept. This shows that building stronger image-text co-embeddings is foundational to improving the Agile Modeling process.


%Furthermore, in the hard concepts, the User-100 models begin to outperform the Crowd-500 models by the third active learning round, despite having one-fifth the amount of training data.
 
%This finding suggests that for difficult, nuanced concepts, a domain-expert centered process is generally more efficient in training image classifiers than using the crowd. 



%Furthermore, in the hard concepts, the User-100 models begin to outperform the Crowd-500 models by the third active learning round, despite having one-fifth the amount of training data. This finding suggests that for difficult, nuanced concepts, a domain-expert centered process is generally more efficient in training image classifiers than using the crowd. 
% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{c|c|c|c|c|c|c}
%          Model & Initial & AL-1 & AL-2 & AL-3 & AL-4 & AL-5  \\
%           \hline
%          Agile (all) &  0. & 0. & 0. & 0. & 0. & 0.  \\
%          Crowd  & 0. & 0. & 0. & 0. & 0. & 0.  \\
%          Crowd$\times5$  & 0. & 0. & 0. & 0. & 0. & 0.  \\
%         \hline
%          Agile (top4) &  0.65 & 0.69 & 0.74 & 0.75 & 0.77 & 0.76  \\
%          Crowd  & 0.67 & 0.73 & 0.76 & 0.77 & 0.78 & 0.78  \\
%          Crowd$\times5$  & 0.69 & 0.77 & 0.79 & 0.80 & 0.80 & 0.80  \\
%          \hline
%          Agile (bot4) &  0.42 & {0.48} & {0.51} & {0.53} & 0.55 & \textbf{0.57}  \\
%          Crowd  & 0.45 & 0.46 & 0.47 & 0.50 & 0.53 & 0.53  \\
%          Crowd$\times5$  & \textbf{0.48} & \textbf{0.51} & \textbf{0.54} & \textbf{0.55} & \textbf{0.56} & 0.55  \\

        
         
%     \end{tabular}
%     \caption{Results for crowd versus agile}
%     \label{tab:crowd_vs agile}
% \end{table}


% \otilia{Eddie, can you please describe this? Including discussion of template creation, time, cost.} 

% A key insight of Agile Modeling is to understand the value of using users. To test this insight, we conduct a series of experiments that test how the performance of our Agile Modeling solution changes when users are replaced with crowd workers. 
% \paragraph{Replacing users with crowd workers.} We replace any rating done by the user in our solution with a crowd worker. Crowd workers read task instructions created by the users, who noted difficult cases that they found during labeling. These instructions and the entire task design can be found in supplementary. Each image is sent to three crowd workers and the majority vote is used as the label. As shown in \kenji{link}, we find that the final model AUPR on average decreased from 0.68 to 0.64, a relative decrease of 6\%.

% However, since the crowd is scalable, we replicate the experiment above, but each initial model and AL round sends 5 times as many images to be rated. As shown in \kenji{link}, we find that the final model on average reached parity with the user model.
% Next, we analyze the performance of crowd labelers co-operatively working with users. In this setting we continue the Agile Modeling process from the final model trained by users and perform two further rounds with large batches of 1000 images each.  


\section{Experiments with ImageNet21k}
Our user study validates the Agile Modeling framework on a small number of concepts over a web-scale unlabelled dataset. Now, we confirm that our framework can be effectively applied across a larger number of concepts to achieve significant improvements over zero-shot baselines. Due to the scale of this experiment, we simulate the user annotations using a fully-labeled dataset.

\vspace{1ex}
\noindent\textbf{Experimental setup.}
We use the ImageNet21k dataset~\cite{deng_imagenet_2009} which contains $21$k classes and over $14$M images. Out of these we select a subset of both easy and difficult classes, as described below. Each class corresponds to a binary classification problem as before. We apply the Agile Modeling framework with the ImageNet21k training set as the unlabeled data pool, and the test set for evaluation. Ground-truth class labels included in the dataset simulate a user providing ratings. Since the Agile Modeling process starts at concept definition with no labeled data, we use the class name and its corresponding WordNet~\cite{miller1995wordnet} description as positive text phrases in the text-to-image expansion step.
As before, we use a batch size of $100$ and $5$ rounds of active learning. We use ALIGN embeddings.

\vspace{1ex}
\noindent\textbf{Concept selection.}
We use a subset of $100$ of the $21$k concepts for evaluation. $50$ ``easy" concepts are selected at random from the ImageNet $1000$ class list. Additionally, we aim to replicate the ambiguity and difficulty of our original concepts by carefully selecting 50 further concepts with the following criteria based the WordNet lexicographical hierarchy: (1) $2$-$20$ hyponyms, to ensure visual variety, (2) more than $1$ lemma, to ensure ambiguity, (3) not an animal or plant, which have objective descriptions. Of the $546$ remaining concepts, our $50$ ``hard" concepts are selected at random. The full list of chosen concepts is in Appendix~\ref{appendix:imagenet}.



\begin{figure}[t]
  \centering
  \vspace{-2ex}
   \includegraphics[width=0.9\linewidth]{img/in21k_experiment_all2-notitle.png}
   \vspace{-1em}
   \caption{Model performance per amount of samples on ImageNet21k for both easy and hard classes (AUC PR mean and std error over classes). Each $\bullet$ represents an AL round.}
   \label{fig:in21k-auc-pr}
  \vspace{-3ex}
\end{figure}

\vspace{1ex}
\noindent\textbf{Results.}
In Figure~\ref{fig:in21k-auc-pr} we show the results of applying the Agile Modeling framework to ImageNet21k. We see a similar trend to our user experiments, with significant improvements over zero-shot baselines as well as continued improvement with each active learning round. We further observe that the ``easy" concepts attained higher scores after the Agile Modeling process than the ``hard" concepts. The zero-shot baseline differed significantly between the ``easy" and ``hard" concepts with scores of 0.29 and 0.11, respectively. The equivalent of 30 minutes of human work yields a 20\% boost in AUC PR over the zero-shot baseline.

==> Agile Modeling - arxiv/sections/5_discussion.tex <==
\section{Discussion \& conclusion}
\label{sec:discussion}

We formalized the Agile Modeling problem to turn any visual concept from an idea into a trained image classifier. We promote the notion of incorporating the user-in-the-loop, by supporting users with interactions that do not require any machine learning experience. We show that by using the latest advances in image-text pretrained models, we are able to initialize, train, and perform active learning in just a few minutes, enabling real-time user interaction for rapid model creation in less than 30 minutes.
% Through a set of experiments with $14$ users, each modeling their own concept, we show that our solution is able to quickly learn from users to create high performing classifiers even on difficult concepts. 
% Agile Modeling empowers users to train models without crowd labeling or machine learning expertise, making it possible to label difficult or highly specific concepts.
Via a simple prototype, we demonstrate the value of users over crowd labelers in generating classifiers for subjective user-defined concepts.
% The difference in performance between using CLIP and ALIGN embeddings further suggests that as foundation models improve, so will Agile Modeling. 
% We believe that all parts the system can be improved to be faster and more accurate, including initialization, model training, and active learning.  
% Additionally, we show that our framework is effective even on a larger number of concepts, on a simulated experiment using ImageNet21k.
We hope that our work showcases the opportunities and challenges of Agile Modeling and encourages future efforts.


